Computing Valid p-value for Optimal Changepoint by Selective Inference using Dynamic Programming

There is a vast body of literature related to methods for detecting changepoints (CP). However, less attention has been paid to assessing the statistical reliability of the detected CPs. In this paper, we introduce a novel method to perform statistical inference on the significance of the CPs, estimated by a Dynamic Programming (DP)-based optimal CP detection algorithm. Based on the selective inference (SI) framework, we propose an exact (non-asymptotic) approach to compute valid p-values for testing the significance of the CPs. Although it is well-known that SI has low statistical power because of over-conditioning, we address this disadvantage by introducing parametric programming techniques. Then, we propose an efficient method to conduct SI with the minimum amount of conditioning, leading to high statistical power. We conduct experiments on both synthetic and real-world datasets, through which we offer evidence that our proposed method is more powerful than existing methods, has decent performance in terms of computational efficiency, and provides good results in many practical applications.

==> sec6_remove.tex <==
\section{Real-data Examples} \label{sec:sec6}
\begin{table}[t!]
\centering
\renewcommand{\arraystretch}{1.2}
\caption{Power comparison on real-data.}
\label{tbl:power_comparison_real_data}
{\footnotesize
\begin{tabular}{|l|c|c|c|c|}
\hline
  & SMUCE & OptSeg-SI-oc & BinSeg-SI & OptSeg-SI \\ 
\hline
  $\bm{\cD}_1$ &  0.53 & 0.24  & 0.33 &  \textbf{0.75} \\ 
\hline
  $\bm{\cD}_2$  & 0.62 & 0.27 &  0.32 & \textbf{0.71} \\ 
\hline
\end{tabular}
}
\end{table}


We performed power comparison on real-data. We used \emph{jointseg} package \cite{pierre2014performance} to generate realistic DNA copy number profiles of cancer samples with ``known" truth.
%
Two datasets with 1,000 profiles of length $N=60$ and true $K = 2$ for each were created as follows: \\
$\bullet$ $\bm{\cD}_1$: Resample from GSE11976 with tumor fraction $=$ 1\\
$\bullet$ $\bm{\cD}_2$: Resample from GSE29172 with tumor fraction $=$ 1\\
%
The results are shown in Table \ref{tbl:power_comparison_real_data}.
%
Our proposed OptSeg-SI has higher power than the other methods in all cases.
%
We also applied OptSeg-SI to the Array CGH data provided by \citet{snijders2001assembly} and the Nile data which contains annual flow volume of the Nile river. %at Aswan from 1871 to 1970.
%
All of the results are consistent with \citet{snijders2001assembly, jung2017bayesian}. More details of the results can be found in Appendix \ref{appendix:real_experiments}.

%
%\begin{figure}[t]
%\begin{subfigure}{.49\linewidth}
%  \centering
%  \includegraphics[width=\linewidth]{GM03576_2}  
%  \caption{Choromosomes 1, 2, 3.}
%  \label{fig:sub_choromosomes_1_2_3}
%\end{subfigure}
%\begin{subfigure}{.49\linewidth}
%  \centering
%  \includegraphics[width=\linewidth]{GM03576_21}  
%  \caption{Choromosomes 20, 21, 22.}
%  \label{fig:sub_choromosomes_20_21_22}
%\end{subfigure}
%\caption{Experimental results for cell line GM03576.}
%\label{fig:exp_cgh_GM03576}
%\end{figure}
%
%\begin{figure}[t]
%\begin{subfigure}{.49\linewidth}
%  \centering
%  \includegraphics[width=\linewidth]{GM01750_14}  
%  \caption{Chromosome 14.}
%  \label{fig:sub_chromosome_14}
%\end{subfigure}
%\begin{subfigure}{.49\linewidth}
%  \centering
%  \includegraphics[width=\linewidth]{GM00143_18}  
%  \caption{Choromosomes 17, 18, 19}
%  \label{fig:sub_choromosomes_17_18_19}
%\end{subfigure}
%\caption{Experimental results for cell lines GM00143 and GM01750.}
%\label{fig:exp_cgh_GM00143_GM01750}
%\end{figure}
%
%
%\begin{figure}[t]
%\centering
%\includegraphics[width=0.85\linewidth]{Nile}  
%\caption{Experimental result for Nile data. The changepoint is detected at $28^{\rm th}$ position which indicates there is a change in volume level in year 1899.}
%\label{fig:exp_nile_data}
%\end{figure}






